Insight into particle production mechanisms via angular correlations of identified particles in pp collisions at $\sqrt{s}=7$ TeV

Two-particle angular correlations were measured in pp collisions at $\sqrt{s} = 7$ TeV for pions, kaons, protons, and lambdas, for all particle/anti-particle combinations in the pair. Data for mesons exhibit an expected peak dominated by effects associated with mini-jets and are well reproduced by general purpose Monte Carlo generators. However, for baryon-baryon and anti-baryon--anti-baryon pairs, where both particles have the same baryon number, a near-side anti-correlation structure is observed instead of a peak. This effect is interpreted in the context of baryon production mechanisms in the fragmentation process. It currently presents a challenge to Monte Carlo models and its origin remains an open question.

==> definitions.tex <==
\newcommand{\Pt}{$p_{\rm{T}}$}
\newcommand{\pt}{$p_{\rm{T}}$}
\newcommand{\pT}{$p_{\rm{T}}$}
\newcommand{\dndh}{${\rm d}N_{\rm ch}/{\rm d}\eta$}
\newcommand{\dndy}{${\rm d}N_{\rm ch}/{\rm dy}$}
\newcommand{\detadphi}{$\Delta\eta\Delta\varphi$}
\newcommand{\dedx}{$\mathrm{d}E/\mathrm{d}x$}
\newcommand{\ee}{$\rm e^+e^-$}

\newcommand{\Jpsi}{J/$\psi$ }
\newcommand{\degree}{\ensuremath{^\circ}}

\newcommand{\pp}{pp}
\newcommand{\pPb}{p--Pb}
\newcommand{\PbPb}{Pb--Pb}
%\newcommand{\sqr7}{$\sqrt{s}=7$}

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
